Cryptocurrency Portfolio Optimization by Neural Networks

Many cryptocurrency brokers nowadays offer a variety of derivative assets that allow traders to perform hedging or speculation. This paper proposes an effective algorithm based on neural networks to take advantage of these investment products. The proposed algorithm constructs a portfolio that contains a pair of negatively correlated assets. A deep neural network, which outputs the allocation weight of each asset at a time interval, is trained to maximize the Sharpe ratio. A novel loss term is proposed to regulate the network's bias towards a specific asset, thus enforcing the network to learn an allocation strategy that is close to a minimum variance strategy. Extensive experiments were conducted using data collected from Binance spanning 19 months to evaluate the effectiveness of our approach. The backtest results show that the proposed algorithm can produce neural networks that are able to make profits in different market situations.

==> figures/neural_network_introduce.tex <==
% NEURAL NETWORK with coefficients, arrows
\begin{tikzpicture}[x=3.0cm,y=2.0cm]
  \message{^^JNeural network with arrows}
  \readlist\Nnod{2,3,2,1} % array of number of nodes per layer
  \readlist\Cstr{\strut x,f^{(\prev)},f^{(\prev)},\hat{y}} % array of coefficient symbol per layer

  \message{^^J  Layer}
  \foreachitem \N \in \Nnod{ % loop over layers
    \edef\lay{\Ncnt} % alias of index of current layer
    \message{\lay,}
    \pgfmathsetmacro\prev{int(\Ncnt-1)} % number of previous layer
    \foreach \i [evaluate={\y=\N/2-\i; \x=\lay; \n=\nstyle;}] in {1,...,\N}{ % loop over nodes
      
      % NODES
      \node[node \n] (N\lay-\i) at (\x,\y) {$\Cstr[\lay]_{\i}$};
      %\node[circle,inner sep=2] (N\lay-\i') at (\x-0.15,\y) {}; % shifted node
      %\draw[node] (N\lay-\i) circle (\R);
      
      % CONNECTIONS
      \ifnum\lay>1 % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \draw[connect arrow] (N\prev-\j) -- (N\lay-\i);
           %  node[pos=0.5] {\contour{white}{$w_{1,\i}$}}; % connect arrows directly
           % \draw[connect arrow] (N\prev-\j) -- (N\lay-\i'); % connect arrows to shifted node
        }
      \fi % else: nothing to connect first layer
      
    }
  }
  
  % LABELS
  \node[above=5,align=center,mygreen!60!black] at (N1-1.90) {input\\[-0.2em]layer};
  \node[above=2,align=center,myblue!60!black] at (N2-1.90) {hidden layers};
  \node[above=8,align=center,myred!60!black] at (N\Nnodlen-1.90) {output\\[-0.2em]layer};
\end{tikzpicture}


==> figures/pgf-example.tex <==
\begin{tikzpicture}[scale=0.9]
\begin{axis}[axis lines=center,
            xlabel={aika (s)},
            xlabel near ticks,
            ylabel={korkeus (m)},
            ylabel near ticks,
            xmin=0, xmax=6, ymin=0]
\addplot[color=black,
        domain=0:30*sin(30)/(0.5*9.81),
        samples=101]
        {30*sin(30)*x - 0.5*9.81*x^2}
        node[color=black, midway, below]{\ang{30}};
\addplot[color=red,
        domain=0:30*sin(40)/(0.5*9.81),
        samples=101]
        {30*sin(40)*x - 0.5*9.81*x^2}
        node[color=black, midway, below]{\ang{40}};
\addplot[color=green,
        domain=0:30*sin(50)/(0.5*9.81),
        samples=101]
        {30*sin(50)*x - 0.5*9.81*x^2}
        node[color=black, midway, below]{\ang{50}};
\addplot[color=blue,
        domain=0:30*sin(60)/(0.5*9.81),
        samples=101]
        {30*sin(60)*x - 0.5*9.81*x^2}
        node[color=black, midway, below]{\ang{60}};
\end{axis}
\end{tikzpicture}
